GEEvo: Game Economy Generation and Balancing with Evolutionary Algorithms

Game economy design significantly shapes the player experience and progression speed. Modern game economies are becoming increasingly complex and can be very sensitive to even minor numerical adjustments, which may have an unexpected impact on the overall gaming experience. Consequently, thorough manual testing and fine-tuning during development are essential. Unlike existing works that address algorithmic balancing for specific games or genres, this work adopts a more abstract approach, focusing on game balancing through its economy, detached from a specific game. We propose GEEvo (Game Economy Evolution), a framework to generate graph-based game economies and balancing both, newly generated or existing economies. GEEvo uses a two-step approach where evolutionary algorithms are used to first generate an economy and then balance it based on specified objectives, such as generated resources or damage dealt over time. We define different objectives by differently parameterizing the fitness function using data from multiple simulation runs of the economy. To support this, we define a lightweight and flexible game economy simulation framework. Our method is tested and benchmarked with various balancing objectives on a generated dataset, and we conduct a case study evaluating damage balancing for two fictional economies of two popular game character classes.

==> content/buffer.tex <==


%Game Balancing
\begin{itemize}
    \item My paper \cite{rupp_balancing_2023}
    \item Game balance with EA for card game, Volz et al.~\cite{volz_demonstrating_2016}
    % Volz et al. [111] used multi-objective optimization to create balanced cards for the Top Trumps card game (Dubreq, 1978). The goal is to generate a group of unique balanced decks such that there is no dominant strategy to win the game. The surrogate model here is a statistical model that predicts the minimum number of simulation that is needed to have an accurate estimation of the win rate. The results showed that generated decks from surrogate models are as good as normal simulations and require a lot less computational power.
    \item MicroRTS units \cite{sorochan_generating_2022}
    \item Pfau: Dungeons and Replicants \cite{pfau_dungeons_2020}
    \item RaidEnv?
    \item Automated balancing framework with RL (Reis) \cite{reis_automatic_2023}
    \item FPS Weapon balancing through PCG with EA \cite{gravina_constrained_2016}
    % adjusted the surprise search algorithm to maintain quality and not only focus on surprise. They utilized the new algorithm (Constrained Surprise Search) to generate a diverse set of balanced weapons for FPS shooter games.
    \item and many more
\end{itemize}



Game Economies
\begin{itemize}
    \item Game balance (economies) \cite{schreiber_game_2021}
    \item Game design \cite{adams_fundamentals_2014}
    \item Balancing economy abstract framework \cite{ranandeh_beyond_2023}
    \item different economies e.g., in contrast positive sums or F2P mobile games.
\end{itemize} 

Evolutionary Algorithms
\begin{itemize}
    \item EA in games (Togelius) \cite{togelius_evolutionary_2024}
    \item Rogers evolutionary economies \cite{rogers_using_2023}
    \item search based PCG \cite{togelius_search-based_2011}
    \item Controllable procedural map generation via multiobjective evolution \cite{togelius_controllable_2013}
    \item and many more
\end{itemize}



\begin{table}[]
\centering
\caption{Results after balancing attributes for the mage and archer economy compared for two different values of $\alpha$ with the goal to deal the same damage within a given period of time.}
\begin{tabular}{l@{\hspace{2.1mm}}ll@{\hspace{2.1mm}}l|l@{\hspace{2.1mm}}ll@{\hspace{2.1mm}}l}
\toprule
\multicolumn{4}{c}{Result $\alpha$=0.05}  & \multicolumn{4}{|c}{Result $\alpha$=0.01} \\ \midrule
\textbf{Mage}          & $w$  & \multicolumn{1}{|l}{\textbf{Archer}} & $w$  & \textbf{Mage}           & $w$   & \multicolumn{1}{|l}{\textbf{Archer}}       &  $w$ \\ \midrule %\hdashline 
M. Reg.    & 3     & \multicolumn{1}{|l}{A-Speed}     & 2    & M. Reg.     & 2       & \multicolumn{1}{|l}{A-Speed}     & 1 \\
A1 CD      & 1     & \multicolumn{1}{|l}{A1 Prob.}    & 0.88 & A1 CD       & 1       & \multicolumn{1}{|l}{A1 Prob.}    & 0.76 \\
A1 M.      & 3     & \multicolumn{1}{|l}{A1 Dmg.}     & 1    & A1 M.       & 3       & \multicolumn{1}{|l}{A1 Dmg.}     & 2 \\ 
A1 Dmg.    & 3     & \multicolumn{1}{|l}{A2 Prob.}    & 0.12 & A1 Dmg.     & 3       & \multicolumn{1}{|l}{A2 Prob.}    & 0.24 \\
A2 CD      & 3     & \multicolumn{1}{|l}{A2 Dmg.}     & 3    & A2 CD       & 2       & \multicolumn{1}{|l}{A2 Dmg.}     & 2 \\
A2 M.      & 2     & \multicolumn{1}{|l}{}            &      & A2 M.       & 2       & \multicolumn{1}{|l}{}            &   \\
A2 Dmg.    & 3     & \multicolumn{1}{|l}{}            &      & A2 Dmg.     & 3       & \multicolumn{1}{|l}{}            &   \\ \midrule  \midrule
\addlinespace[2pt]
\textbf{$\sum$ Dmg.} & 55    &   \multicolumn{2}{|c|}{53.8$\pm$4.8}      & \multicolumn{2}{c}{60} &   \multicolumn{2}{|c}{60$\pm$0} \\ \midrule

\multicolumn{1}{l}{\textbf{Fitness}} &  \multicolumn{2}{c}{0.95 + $\alpha$} &   &   \multicolumn{4}{c}{1.0 + $\alpha$}
\vspace{-1.5mm}
\label{tab:mage-archer}
\end{tabular}
\end{table}

==> content/recovery.tex <==

\section{Introduction}

%The success of a game, board games such as video games, depends heavily on the design and balancing of its internal economy. This economy defines how virtual resources are created and can be transitioned to other resources. In addition, a well-designed economy incentivizes players to engage in certain behaviors to increase their virtual progress and to keep playing the game.

Games, be they board games or video games, that feel unbalanced are unsatisfactory for players, leading to boredom or frustration and players will quit playing~\cite{becker_what_2020}. A game's balancing is thereby heavily influenced by the design and balancing of its internal economy which defines how virtual resources are created and can be transitioned to other resources.
A well-designed economy is a powerful system, incentivizing players to engage in certain behaviors to increase their virtual progress and to keep playing the game~\cite{schreiber_game_2021,adams_fundamentals_2014}.
This concept is present in many game genres such as in simulation games like \emph{Catan} or \emph{Factorio} (transitions of resources like e.g., wood or iron), first person shooters (health points and its relation to weapon damage), role playing games like \emph{The Legend of Zelda} or \emph{World of Warcraft} (e.g., mana and ability cool downs), or the players' most valuable resource: their time.
Defining how many resources are generated or required for each transition has a strong impact on the entire system and is therefore often difficult to configure to achieve overall balance. Even a small change in these quantities can have large and sometimes unforeseen effects on the overall economic behavior and therefore on the entire playing experience. This is particularly the case when it comes to probabilistic mechanisms within the economic system, such as the type and amount of resource creation based on e.g., a dice roll. For this reason, the design and balancing of game economies requires a lot of manual work, testing and fine-tuning in the development process~\cite{schreiber_game_2021}.

%With this work we ask the question if we can optimize an existing or generated game economy algorithmically to satisfy different balancing objectives to support game designers in the design and balancing phase. Such an objective can e.g., be the balancing of two different economies to behave comparable (cf. balancing characters) or the counteracting of positive sum economies. 
%Many works have been presented to automatically balance parameters of game content using search-based approaches such as in X. These methods, however, focus on a specific game or genre. In contrast, this work approaches the problem of game balancing by modeling graph-based game economies that formulate the game's internal resource flows at a more abstract level.
%Little work has been presented on the procedural generation of game economies in literature. X propose an evolutionary algorithm (EA) to generate graph-based economies of different complexities for a simulation game.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{content/img/example_sample.png}
  \caption{Example of a generated game economy. Its graph defines how resources are generated (sources) and are transitioned (converters and random gates). Using an evolutionary algorithm, we optimize the economy's weights towards a specified balancing objective with simulated data of the economy.}
  %We simulate the economy to adapt its weights using an EA toward specified balancing goals.}
  \label{fig:sample-economy}
\end{figure}

To support game designers in this important, but time consuming process, this work explores the algorithmic optimization of existing or generated game economies to meet various balancing objectives (e.g., character damage dealing).
Existing works focus on specific games or genres to address game balancing~\cite{volz_demonstrating_2016,sorochan_generating_2022,pfau_dungeons_2020,gravina_constrained_2016,mesentier_silva_evolving_2019}, whereas this research takes a different approach by modeling graph-based game economies at a more abstract level.
Therefore, we propose GEEvo (Game Economy Evolution), a framework including two evolutionary algorithms (EAs) to generate and balance graph-based game economies simulation-driven. Analogous to the work presented in~\cite{rupp_balancing_2023}, we separate the generation and balancing into distinct units, addressing thereby the procedural content generation (PCG) and balancing problem separately.
Little work has been presented on the generation of game economies itself in literature. Rogers et al.~\cite{rogers_using_2023} EA to generate graph-based game economies of different complexities for a simulation game. In this work, however, we address more complex economies including probabilistics for instance. Therefore, we create the \emph{generator}, an EA to controllably generate random yet valid economies and run simulations using a lightweight framework inspired by Machinations\footnote{https://machinations.io/} which is based on the domain-specific language introduced in~\cite{klint_micro-machinations_2013}. With this approach, an economy can flexibly modeled as a graph with nodes representing functional components (cf.~Figure~\ref{fig:sample-economy}).
The \emph{balancer}, the second EA, optimizes then the resource flow by adjusting edge weights in the economy graph.
To assess our method, we evaluate the general performance on a set of generated economies and conduct a case study in balancing the damage output of fictitious economies of a mage and an archer. The Python code, along with the simulation framework, can be found on GitHub\footnote{The link to Github is anonymized for double-blind review.}.
Our contributions are:
\begin{itemize}
    \item The \emph{balancer}: An evolutionary algorithm to balance graph-based game economies simulation-driven by optimizing its weights towards different objectives. %such as comparable resource transitions.
    \item The \emph{generator}: An evolutionary algorithm for creating random but valid game economy graphs that are controllable in terms of output size and components.
    \item A lightweight framework to simulate game economies.
    \item A study to evaluate the balancing of generated economies with respect to different balancing objectives. In it, we demonstrate balancing using an example setting of damage dealing for a mage and an archer.
\end{itemize}

The paper is structured as follows: We give an overview of related work in Section~\ref{sec:related-word} and the method in Section~\ref{sec:method}. The latter includes the description of the economy simulation~framework~(\ref{sec:framework}), the generator~(\ref{sec:ea-gen}) and balancer~(\ref{sec:ea-balance}).
Experiments and results are described in Section~\ref{sec:experiments}, the discussion and limitations in~\ref{sec:discussion}, and the conclusion and future work in~\ref{sec:conclusion}.

%What are game economies?
%Why is balancing important?
%Can we generate and them with PCG and balance them afterwards?

%Positive sum economies
%Example: little change can have big impact



\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{content/img/process.png}
  \caption{The process with GEEvo is twofold: in step 1 a game designer models an existing game economy as graph with our framework. New economy graph can also be created based on a given configuration with our generator. In Step 2 is an iterative process where the weights of the graph are optimized with the balancer toward a given objective. After each iteration, the designer can evaluate the optimized weights. If necessary, the balancer can be reconfigured for further iterations, for example to enable the definition of specific weights for a particular narrative context as static or to increase the impact of probabilistics within the economy.
  }
  %We simulate the economy to adapt its weights using an EA toward specified balancing goals.}
  \label{fig:process}
\end{figure}


\section{Related Work}
\label{sec:related-word}

Game economies have been studied in depth in the basic books~\cite{schreiber_game_2021} and~\cite{adams_fundamentals_2014}. A game's economy massively contributes to the overall game experience including its balancing and how fast players progress in the game. Especially through balancing the progress, free to play games use players' impatience for monetization~\cite{evans_economics_2016}.
Klint et al.~\cite{klint_micro-machinations_2013} introduce a domain specific language to flexibly model game economies as a graph which has been adapted further in~\cite{vanrozen_adapting}. The authors therefore introduce different node types which create and transition resources. Based on the proposed design, we implement a more lightweight implementation as we focus on the balancing with EAs. A conceptual framework to get a faster and better understanding when creating and balancing game economies is proposed in~\cite{ranandeh_beyond_2023}.

In this work, we use EAs for game economy generation and balancing. In the area of games research, EAs are used extensively e.g., for game balancing~\cite{volz_demonstrating_2016,sorochan_generating_2022,gravina_constrained_2016,morosan_automated_2017}, playing a game~\cite{gaina_rolling_2017}, or procedural generation of content (PCG) such as levels~\cite{togelius_search-based_2011,togelius_controllable_2013,shaker_evolving_2012}, scenarios~\cite{gerhold_computer_2023}, narratives~\cite{alvarez_tropetwist_2022}, rules~\cite{cook_mechanic_2013}, or textures~\cite{wiens_gentropy_2002} (cf. search-based PCG). A detailed and actual survey about the usage of EAs for games is given by Togelius et al. in~\cite{togelius_evolutionary_2024}.

Whereas this work aims at balancing a game through its economy from a more abstract perspective, many works focus on a single game or genre to adjust game unit parameters or create new units using an EA. Volz et al. \cite{volz_demonstrating_2016} create balanced decks for a card game using an evolutionary multi-object optimization strategy. To estimate a deck's win rate, the authors also use a simulation-driven approach but supported by a statistical surrogate model. In~\cite{mesentier_silva_evolving_2019} an EA is introduced to balance card attributes for the game \emph{Hearthstone}.
Gravina et al.~\cite{gravina_constrained_2016} introduce the Constraint Surprise Search, a divergent evolutionary search method, to generate sets of diverse and balanced weapons for first person shooter (FPS) games.
Morosan et al.~\cite{morosan_automated_2017} use an EA to balance a real time strategy game (RTS) and Sorochan et al.~\cite{sorochan_generating_2022} to generate new and balanced units for an RTS game.
Another approach to balancing a game can be done through procedural generation of the game map as shown for FPS games in~\cite{lanzi_evolving_2014} and~\cite{lara-cabrera_balance_2014}. Automated game balancing, however, is not limited to EAs. In~\cite{pfau_dungeons_2020} data-driven deep player behavior models are created to replicate human behavior to adapt game parameters. Furthermore, reinforcement learning is also popular e.g., for difficulty balancing~\cite{reis_automatic_2023} or the generation of balanced levels~\cite{rupp_balancing_2023}. We build on the idea presented in this paper to split the generation and balancing step into two separate units and calculating the fitness in a simulation-driven manner.

Little work has been presented on the automated generation or balancing of game economies itself. In~\cite{rogers_using_2023} the generation of graph-based game economies using an EA is proposed. The authors thereby focus on the generation of economies with different perceived complexity levels and proof their results alongside with a user study. In their implementation the economy is represented by a tree structure where each resource is always forwarded to a resource conversion. In contrast to this work, we focus on the \emph{balancing} of the economy and allow for more complex economies including probabilities or supporting circles within in the graph.

Besides balancing and game economies, EAs in the context of games are applied for PCG tasks~\cite{shaker_procedural_2016} such as the generation of levels. A taxonomy and survey is given in~\cite{togelius_search-based_2011}. \cite{togelius_controllable_2013} proposes an EA to generate levels for an RTS game using a controllable multi-object approach.
Search-based methods like EAs, however, have a high dependency on randomness and are also computationally intensive at inference. Therefore, \cite{khalifa_mutation_2022} introduces mutation models that combine evolution with machine learning to enable faster generation of game levels. As a different approach, the PCGRL framework~\cite{khalifa_pcgrl_2020} proposes to use reinforcement learning for level generation, since after once a model has been trained, the inference is fast.


%\item narrative graphs \cite{alvarez_tropetwist_2022}


\section{Method}
\label{sec:method}
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{content/img/architecture.png}
    \caption{The architecture of our method at a glance, consisting of two EAs: one for economy balancing and one for the random but constraint-based generation of economies. The generator is controllable in terms of generating graphs of specific sizes with given amounts of distinct node types. These generated economies can be the input for the balancer, however, already existing economies can be fed in as well. The balancer adjusts the weights based on fitness functions to optimize the weights on the edges by simulating the economy.}
    \label{fig:architecture}
\end{figure*}


\begin{table*}
    \centering
    \caption{Overview of the different node types and their constraints to create valid game economies.}
    \begin{tabular}{|l|c|c|c|c|l|l|l|} \hline 
         \textbf{Node types $T$} &  \textbf{max in}&  \textbf{max out}&  \textbf{min out}&\textbf{min in}&\textbf{allowed inputs} & \textbf{allowed outputs} & \textbf{color} \\ \hline 
         Source&  0&  3&    1&0&-&Pool, Random Gate &green\\ \hline 
         Random Gate& 1& 3&   2&1&Source, Converter&Pool, Converter&red\\ \hline 
         Pool& 2& 3&   1&1&Source, Random Gate, Converter&Converter, Drain &blue\\ \hline 
         Converter& 3& 1&   1&1&Pool, Random Gate&Pool, Random Gate&yellow\\ \hline 
         Drain& 2& 0&   0&1&Pool&- &orange\\ \hline
    \end{tabular}
    \label{tab:node-types}
\end{table*}


The architecture of our method is shown in Figure~\ref{fig:architecture}. It consists of two EAs, one for the constraint-based generation of game economies and a second one for the balancing of an economy's weights according to a given balancing objective. As applied in~\cite{rupp_balancing_2023}, we also separate the generation and balancing processes into two separated units which results in better performances of both.
Additionally, the encapsulation allows the application of the balancing to already existing economies for instance.
The economy generator is controllable in terms of the economy's graph's size and the distinct number of each node type. The balancer simulates the economy for $n$ time steps to calculate the fitness of its current weights.
%The fitness function differs depending on the balancing goal.

Before we describe both EAs in detail in Sections~\ref{sec:ea-gen} and~\ref{sec:ea-balance} including an overview of the different fitness functions, we describe our economy simulation framework and its application.


\subsection{Game Economy Simulation Framework}
\label{sec:framework}


A game economy can be considered as a directed graph which defines how resources of different types are generated and transitioned to other resource types. In this work, we only deal with fixed economic systems, where all resources come from the economy itself.
In this context, nodes in that graph represent different functional components such as the creation of resources or conversion to different types. Weights on the edges describe how many resources flow from one node to the adjacent one. Depending on the node type, the weights are absolute values or probabilities.

Our framework defines five different node types. In order to generate valid and executable economy graphs we additionally define constraints for each node type e.g., to which node type each may be connected (Table~\ref{tab:node-types}). The values for maximum (max) and minimum (min) output sizes are each chosen to keep the economies more manageable. However, these values could also be changed to allow for more complex economies (e.g., increase max output).

\paragraph{Source} Sources are entry points creating resources and adding them to the economy.
\paragraph{Random gate} A random gate distributes incoming resources based on the probabilistic weights of its outgoing edges. It must be ensured that the sum of the weights of all outgoing edges equals one. This can be used to model e.g., critical attacks or random drops.
\paragraph{Pools and fixed Pools} Pool nodes have an intern memory to store incoming resources. They serve as buffers for outputs from sources, random gates or converters or as end points of the economy. For the analysis of the economy we can monitor the fluctuations of the resources within pools over time. Fixed pools, a subform of a pool buffer a maximum of the number of resources equal to the highest outgoing weight. This is particularly useful when modeling ability cooldowns.
\paragraph{Converter} A converter transitions one or multiple incoming resources to one outgoing resource.
\paragraph{Drain} Drains permanently remove resources from the economy. As with pools, it is possible to monitor how many resources have been drained by a distinct one over time.


An example of how to model an existing economy from the sandbox game Minecraft~\cite{mojang_mincraft_2011} is given in Figure~\ref{fig:example-economy}. It shows the torch crafting process in an automation setting where per time step specific amounts of resources are added to the economy via sources. Using pool and converter nodes we can define this economy for torches from wood and coal sources. While coal can be directly used for crafting torches, the wood resource has to be converted to sticks first. According to the original implementation\footnote{https://www.minecraft-crafting.net/} the conversion to sticks yields four sticks per two wood entities. In this example, other resources such as the time to collect resources or the need for a crafting table for resource conversion are neglected.

\begin{figure*}
\centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{content/img/torch.png}
    \caption{Example economy from the game Minecraft for crafting torches from basic wood and coal resources.}
    \label{fig:example-economy}
    \vspace{0.8cm}
  \end{subfigure} 
  \begin{subfigure}[b]{0.5\textwidth}
  \centering
    \begin{subfigure}{0.95\textwidth}
        \centering
      \includegraphics[width=\textwidth]{content/img/torch_sim1.png}
      \caption{Simulation 1: $X=1$ (original value).}
      \label{fig:example-economy-sim1}
    \end{subfigure}
    \begin{subfigure}{0.95\textwidth}
    \centering
      \includegraphics[width=\textwidth]{content/img/torch_sim2.png}
      \caption{Simulation 2: $X=2$ (value for demonstration).}
      \label{fig:example-economy-sim2}
    \end{subfigure}
  \end{subfigure}
  \caption{Example of a game economy using the proposed framework and two simulations of it, each with a different configuration. The graph (a) shows the economy from the game Minecraft to craft torches from wood and coal in an automation setting. (b) and (c) show the monitoring of the pool nodes simulating the economy in (a). By only changing the amount of coal needed to craft torches, the entire economy behaves differently.}
\end{figure*}


\emph{Execution of Game Economy Simulations:}
The directed graph $G$ of a game economy can be denoted as $G=(V,E)$, where $V$ are its vertices (nodes) and $E$ are the edges connecting vertices. For each vertex $v_i \in V$ a subset $A^{v_i} \subset E$ exists containing all outgoing edges. The types of all allowed node types (such as source or pool) are described in the set $T$ (cf. Table~\ref{tab:node-types}).
The execution of the graph economy is then done recursively. For each $v_i$ all edges $e_j \in A^{v_i}$ are executed by a function $f_{\tau}(v_i, e_j),\, \tau \in T$
%with the weight of the edge $w_{e_j},\, e \in A^{v_i}$ 
, $f_{\tau}$ respectively to the type $\tau$ of $v_i$.

We plot two example courses of simulations with different weights of the economy in Figure~\ref{fig:example-economy} in the Figures~\ref{fig:example-economy-sim1} and~\ref{fig:example-economy-sim2}. For this example we assume both resources, wood and coal, to create one of each per time step. By changing the needed amount $X$ for coal to converse coal and sticks to torches this examples demonstrates how small changes to a single weight can impact the whole economy. While e.g., for $X=1$ the amount of torches grows linearly per time step; for $X=2$ it is gradual. Also the curve progressions of available wood and coal is different.


\subsection{Evolutionary Generation of Game Economies}
\label{sec:ea-gen}
The generator implements a greedy mutation-driven strategy to generate valid and directed game economy graphs for the framework described in Section~\ref{sec:framework}. A valid economy graph is given if all constraints listed in Table~\ref{tab:node-types} apply and it is weakly connected. We design the generator to be controllable in terms of the number and type of vertices that will make up the graph to be generated, e.g., the generation of an economy consisting of three sources, two random gates, one converter and four pools.
The execution of the algorithm stops if a valid graph has been found or a maximum of allowed steps is exceeded.


\subsubsection{Initialization and Population} During initialization, all vertices defined in the external configuration are initialized depending on their type. The population consists of only one individual, which represents the edge list of the graph. In the first generation it is empty.
\subsubsection{Mutations} Mutations are the driving force to evolve the graph.
Since the performance is good enough with this approach (cf. Section~\ref{sec:ea-gen}), we abstain the implementation of a crossover. In each generation, two vertices are randomly selected to add an edge. If this edge is allowed due to the constraints, it is added to the individual, otherwise it is not. This simple and greedy approach may get stuck, since at some point the graph is still not valid and no valid edges are allowed anymore. To address this shortcoming, in each generation a previously created edge is randomly removed from the individual with a certain probability.
\subsubsection{Fitness function} The fitness function (Eq.~\ref{eq:fitness}) embeds the constraints to ensure the validity of the graph $G$ with $m$ vertices $V$. It creates the graph based on the created edges and sums up for each vertex $v \in V$ how many constraints are not satisfied. We count every constraint that is not met with an auxiliary function $validate(v)$. The function is defined in the interval $[0,\infty)$, where 0 represents the maximum fitness of an individual; to achieve maximal fitness the function must therefore be minimized:

\begin{equation}
\label{eq:fitness}
fitness(G) = \sum_{v\,\in\,V}{\, validate(v_i) }
\end{equation}


\subsection{Evolutionary Balancing of Game Economies}
\label{sec:ea-balance}

The balancer optimizes the weights of one or multiple economies towards a balancing objective which is expressed via a fitness function (cf. Section~\ref{sec:fitness-functions}). We define the balancer by defining a population consisting of individuals and iteratively optimizing this population through crossover and mutations over multiple generations. Following crossover and mutations, the population undergoes sorting based on fitness, retaining only individuals up to the population size for the subsequent generation.
The algorithm terminates either when the fitness is at its best for a single individual or the maximum number of generations is exceeded. 

\subsubsection{Individuals and population} A population consists of $n$ individuals where each represents all weights of an economy. It can be thought of as a list where each weight's index is mapped to the same index of the graph's edge list. For the case when balancing two economies at once, an individual consists of the two weights lists of the respective economies. At the initialization of an individual its weights are set randomly where all values must be greater than 0. 

\subsubsection{Crossover}
In each generation all individuals of the current population are paired randomly for crossover. For each pair, we iterate over both individuals' $k$ and $l$ weights $w_{ki}, \, w_{li}$ simultaneously and apply one of four randomly selected operations, each with equal probability. The four operations for the new weight at index $i$ are choosing $w_{ki}$ or $w_{li}$ directly, $w_{ki} + w_{li}$ or, $w_{ki} - w_{li}$. After crossover, two individuals each produce a new child individual.

%By applying a one-point crossover, each parental pair produces two new individuals. First, the splitting point is determined randomly. Second, at this point both parents are separated and reunited with the other part of the other parent and vice versa.

\subsubsection{Mutations}
For each mutation a random individual is selected from the population and a random weight is chosen. This weight is then modified by either adding or subtracting the random number by 0.5 each. If subtracting would yield a value $<0$ it is set to 1. 
%To sustainably maintain the population at a diverse level of genomes, we add a new random individual with a 1\% change.

\subsubsection{Fitness functions}
\label{sec:fitness-functions}
With the fitness function we define the goal towards which an economy should be balanced. All fitness is computed by observing the state $s_{t}^{p_j}$ (the amount of contained resources) of one or multiple pool nodes $p_j \in P, P \subset V$ at a selected time step $t, t \leq n$ within the $[1,n]$ steps of a simulated economy. 
%Observing multiple time steps within a single simulation is possible, depending on the fitness function $f$, as well.
To mitigate randomness, we run each simulation with the same weights $m$-times (see Section~\ref{sec:m-sim}).
\paragraph{Balancing a resource to an absolute value} This function (Eq.~\ref{eq:f1}) is motivated by adapting the weights of an economy so that a selected $p_j$ equals a given value $x$ after a fixed number of time steps $n$. A use case for instance is to balance the economy to be capable of producing a distinct amount ($x$) of a resource ($p_j$) within a given time period ($n$). Such a resource can e.g., be coal or damage points, depending on the setting.
Since $s_{t}^{p_j}$ is based on simulations including randomness, we add an additional parameter $\alpha$ as a threshold value to the average so that the algorithm can also terminate at values close to the maximum fitness. As we will later explore (cf. Section~\ref{sec:case-study}), the configuration of this parameter is further important to control the influence of randomness in an economy when balancing.
Equation~\ref{eq:f1} is defined in the interval $[0,1+\alpha]$, where $1+\alpha$ represents the maximum fitness of an individual. The auxiliary function $prop$ (Eq.~\ref{eq:f}) computes the proportion of $x$ and $s_{t}^{p_j}$.


\begin{equation}
\label{eq:f1}
f_1(s_{t}^{p_j}, x) = 
    \alpha + \frac{1}{m} \sum\limits_{i=1}^{m} prop(s_{ti}^{p_j},x), \quad p_j \in P
\end{equation}

\begin{equation}
\label{eq:f}
prop(s_{t}^{p_j}, x) = 
\begin{cases} 
     s_{ti}^{p_j} \cdot \cfrac{1}{x},\quad x > 0 & \text{if } x > s_{ti}^{p_j} \\[9pt]
     x \cdot \cfrac{1}{s_{ti}^{p_j}},\quad s_{ti}^{p_j} > 0 & \text{if } x \leq s_{ti}^{p_j}
\end{cases}
\end{equation}


%\begin{equation}
%\label{eq:f1}
%f_1(s_{t}^{p_j}, x) = \frac{1}{m} \sum_{i=1}^{m}{|\, 1 - s_{ti}^{p_j} cdot \frac{1}{x}\,|}, \quad p_j \in P,\; x > 0 
%\end{equation}

To balance two resources $s_{t}^{p_j}$ and $s_{t}^{p_k}$ within the same economy instead of a single absolute value we can use Equation.~\ref{eq:f1}, but with a different parametrization: $f_1(s_{t}^{p_j}, s_{t}^{p_k}), p_j,p_k \in P$

%Function $f_2$ is an adaption of  :

%\begin{equation}
%\label{eq:f2}
%f_2(s_{t}^{p_j}, s_{t}^{p_k}) = f_1(s_{t}^{p_j}, s_{t}^{p_k}), \quad p_j,p_k \in P
%\end{equation}


\paragraph{Balancing two resources of different economies to the same value} Function $f_2$ parameterizes Eq.~\ref{eq:f1} to balance two resources of two different economies $\theta$ and $\phi$. We apply this function in the case study in Section~\ref{sec:case-study} to balance the dealt damage of a mage and an archer class within the same time period:

\begin{equation}
\label{eq:f3}
f_2(s_{t}^{p_j}, s_{t}^{p_k}) = f_1(s_{t}^{p_j}, s_{t}^{p_k}), \quad p_j \in P_\theta, \;p_k \in P_\phi
\end{equation}

%\paragraph{Balancing a resource}

%\subsection{How often to simulate?}
\label{sec:m-sim}

\section{Experiments and Results}
\label{sec:experiments}
The evaluation is twofold: First, we investigate on the general performance of the generator and second, the balancer including a case study.

\subsection{Evaluation of Game Economy Generation}
To evaluate the generator we create a set of 200 economy graphs with a number of nodes in the range of 5 to 20. Also the distribution of different node types is randomly varied. Within 50k iterations, the algorithm could generate valid graphs according to the constraints and the external configuration in 97\% of cases. The generated dataset therefore consists of 194 graphs.
The median number of iterations required to complete is 641 (90\% quantile: 9354), the median running time is 25~ms (90\% quantile: 296 ms)\footnote{We use for all experiments an Intel Core i7-9700 with 3 GHz.}. 
%In comparison the EA introduced in~\cite{rogers_using_2023} has a computation time, depending on the complexity of the economy, in the average range of 48.83 ms to 614.47 ms.
%On average, a graph was generated in 2420 iterations, resulting in an average execution time of 86.5 ms.

We use this set of economy graphs for the evaluation of the balancer with different balancing objectives.
A generated example economy consisting of seven nodes is shown in Figure~\ref{fig:sample-economy}. In this example the weights are initialized randomly. They are to be balanced in experiments in the next section.

\subsection{Evaluation of Game Economy Balancing}

\subsubsection{General Performance with different balancing objectives}

To assess the balancer's overall performance, we apply it to the previously generated dataset, focusing on balancing a randomly selected pool of an economy to a specific value after a defined number of simulation steps. To test the algorithm's adaptability to varied values, both the number of simulation steps and the specific target value are randomly chosen within the intervals $[10,30]$ and $[20,100]$, respectively. An example would be balancing Pool-5 in Figure 1 to a value of 28 after 16 simulation steps.
Therefore, we employ the fitness function (Eq.~\ref{eq:f1}) introduced earlier.
%which is also the basis for Equation~\ref{eq:f3}.
Given the probabilistic nature of random gates, achieving maximum fitness is often impossible; hence, we compare the results for different values of $\alpha$. The timeout for the algorithm to stop is set to 500 iterations. The size of the population is set to 20 and we run ten simulations with the same weights each generation for each individual. This results in 300 simulation runs per generation alone.

The results are shown in Table~\ref{tab:gen-performance}. The proportions of balanced and initially balanced economies differs depending on $\alpha$. 

%\begin{figure}
%  \begin{subfigure}[b]{0.5\textwidth}
%    \begin{subfigure}{\textwidth}
%      \includegraphics[width=\textwidth]{content/img/init_fitness.png}
%      \caption{Distribution of the initial fitness.}
%      \label{fig:example-economy-sim1}
%    \end{subfigure}
%    \begin{subfigure}{\textwidth}
%      \includegraphics[width=\textwidth]{content/img/fitness.png}
%      \caption{Distribution of the fitness after applying the the EA for balancing.}
%      \label{fig:example-economy-sim2}
%    \end{subfigure}
%  \end{subfigure}
%\includegraphics[width=1\linewidth]{content/img/general_performance.png}
%  \caption{Results for balancing the generated dataset of economy graphs using fitness function 1 (Eq.~\ref{eq:f1}). To demonstrate generalization of the method, a random pool is chosen from each economy which is to be balanced toward a random value within a random amount of simulation steps. The initial fitness is shown in  blue, the fitness after balancing in green.}
%  \label{fig:res-balancing}
%\end{figure}

%The distributions of the fitness before and after balancing are shown in Figure~\ref{fig:res-balancing}. A proportion of 15.5\% was already balanced at initialization. After the application of the balancer, 79,6\% could be balanced toward the given constraints. In 92.8\% of cases it could at least improve the fitness. The median number of iterations is at 21 (90\% percentile: 2000) resulting in a median execution time of 8.02 s (90\% quantile 394.25 s). 



\begin{table}
    \centering
    \caption{Results for balancing the generated dataset of economy graphs using fitness function 1 (Eq.~\ref{eq:f1}) towards different values of $\alpha$.}
    \begin{tabular}{l|ccc}
            &  $\alpha=0.05$&  $\alpha=0.01$& $\alpha=0.0$\\ \hline
         \textbf{Balanced (\%)} &  93.3&  83& 58.8\\
         \textbf{Improved (\%)} & 77.3& 88.7&94.8\\
         \textbf{Initial balanced (\%)} &  27.3&  8.8& 2.5\\
         \textbf{Median generations} &  1&  7& 196\\
         %\textbf{Generations (P90)} &  72,1&  299 & 299\\
         \textbf{Median execution time (s)} &  18,4&  66& 703.2\\
         %\textbf{Execution time (P90, s)} &  216,7&  4022,1& 10772,8\\
    \end{tabular}
    \label{tab:gen-performance}
\end{table}


\subsubsection{Case study: Balancing a Mage with an Archer}
\label{sec:case-study}
Many game genres (e.g., MOBA: Multiplayer Online Battle Arena) offer players the opportunity to choose from different characters, each assigned to specific classes.
While each character has a unique game design, characters of the same class have a similar play style. The different character designs offer players various strategies to win the game. However, in order for a game to be balanced, it is necessary to ensure that different strategies, if played well, are viable~\cite{schreiber_game_2021}.

In this case study, we examine our method for its ability to balance two different existing economies, using two popular classes as an example: a mage and an archer. Both classes have different economies and we want to have a similar maximal damage output for both after a certain period of time. Therefore, we use the parametrization in (Eq.~\ref{eq:f3}).
Both economy graphs are shown in Figure~\ref{fig:economies-case-study}.
The mage's game design is based on casting two different abilities (Fig.~\ref{fig:economy-mage}). Each ability has a specific mana cost, a cooldown, and a value for the damage it deals. Mana is generated at each time step. So there are seven values which need to be balanced accordingly: the cooldowns, mana costs, and damage values for both abilities; as well as the overall amount of mana regenerated per time step.
In contrast, the archer is designed to perform attacks that have a cooldown based on its attack speed (Fig.~\ref{fig:economy-adc}). Each attack has a chance to deal additional damage (cf. critical damage). In this economy five values can be adjusted for balancing: the probabilities for a normal attack and critical damage, the damage values for both, and the attack speed.


We run the balancer with two different values for the fitness threshold $\alpha$, each time with the same seed. To mitigate randomness we run 10 simulation with a length of 30 time steps per generation and a population size of 10.
The algorithm terminates after two generations $\alpha=0.9$ with a total computation time of 1.4 seconds. For $\alpha=0.99$ the algorithm terminates after 25 generations in 16.6 seconds.


\begin{table}[]
\centering
\caption{Results after balancing attributes for the mage and archer economy compared for two different values of $\alpha$ with the goal to deal the same damage within a given period of time.}
\begin{tabular}{l@{\hspace{2mm}}ll@{\hspace{2mm}}l|l@{\hspace{2mm}}ll@{\hspace{2mm}}l}
\hline
\multicolumn{4}{c|}{Result $\alpha$=0.1}  & \multicolumn{4}{|c}{Result $\alpha$=0.01} \\ \hline
\textbf{Mage}          & $w$ & \multicolumn{1}{:l}{\textbf{Archer}} & $w$  & \textbf{Mage}           & $w$   & \multicolumn{1}{:l}{\textbf{Archer}}       &  $w$ \\ \hdashline 
M. Reg.    & 3     & \multicolumn{1}{:l}{A-Speed}     & 2    & M. Reg.     & 2       & \multicolumn{1}{:l}{A-Speed}     & 1 \\
A1 CD      & 1     & \multicolumn{1}{:l}{A1 Prob.}    & 0.88 & A1 CD       & 1       & \multicolumn{1}{:l}{A1 Prob.}    & 0.76 \\
A1 M.      & 3     & \multicolumn{1}{:l}{A1 Dmg.}     & 1    & A1 M.       & 3       & \multicolumn{1}{:l}{A1 Dmg.}     & 2 \\
A1 Dmg.    & 3     & \multicolumn{1}{:l}{A2 Prob.}    & 0.12 & A1 Dmg.     & 3       & \multicolumn{1}{:l}{A2 Prob.}    & 0.24 \\
A2 CD      & 3     & \multicolumn{1}{:l}{A2 Dmg.}     & 3    & A2 CD       & 2       & \multicolumn{1}{:l}{A2 Dmg.}     & 2 \\
A2 M.      & 2     & \multicolumn{1}{:l}{}            &      & A2 M.       & 2       & \multicolumn{1}{:l}{}            &   \\
A2 Dmg.    & 3     & \multicolumn{1}{:l}{}            &      & A2 Dmg.     & 3       & \multicolumn{1}{:l}{}            &   \\ \hline
\addlinespace
\textbf{$\sum$ Dmg.} & 55    &   \multicolumn{2}{:c|}{51.8$\pm$4.8}      & \multicolumn{2}{:c}{60} &   \multicolumn{2}{:c}{60$\pm$0} \\
\textbf{Fitness} &  \multicolumn{2}{c}{0.92 + $\alpha$} &   &   \multicolumn{4}{c}{1.0 + $\alpha$} 
\label{tab:mage-archer}
\end{tabular}
\end{table}

Results of the found attributes (weights) are displayed in Table~\ref{tab:mage-archer}.
For both runs, the balancer finds a solution and terminates within the permitted number of generations. The weights found for the mage are both comparable, whereas those for the archer differ mainly for the probabilistic values for a critical hit. With $\alpha=0.1$, a critical hit (A2) with a change of 12\% would cause 3 damage, a normal attack only 1 damage. For $\alpha=0.01$, the probabilities for a critical hit are irrelevant, as the balancer has equalized the damage for both cases.



\begin{figure*}
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{content/img/mage.png}
    \caption{The mage's economy graph. Seven values can be balanced accordingly: the cooldowns (CD), mana costs (Cost A1, A2), and damage values (Dmg.) for both abilities (A1 and A2); as well as the overall amount of mana regenerated per time step.}
    \label{fig:economy-mage}
  \end{subfigure}
  \hspace{0.5cm}
  \begin{subfigure}[b]{0.45\textwidth}
      \includegraphics[width=\textwidth]{content/img/adc.png}
      \caption{The archer's economy graph: Five values can be balanced accordingly: the overall attack speed, the probabilities (Prob.) to perform a normal or critical attack and the the damage values for each.}
      \label{fig:economy-adc}
    \end{subfigure}
  \caption{Economy graphs for the case study to balance the damage dealing of a mage (a) and an archer (b). The values to be balanced are the weights on the edges. Fixed values are represented by absolute values.}
  \label{fig:economies-case-study}
\end{figure*}

\section{Discussion and Limitations}
\label{sec:discussion}

%\begin{itemize}
%    \item EA generation works, quick and simple
%    \item EA balancing works, however, depends which node to balance, to which value, in which time frame.
%    \item Case study: threshold $\alpha$ configures impact of randomness, discuss two different configs.
%    \item Limitations: Only economy, not player skill, game environment, evaluates the "math". ,help to find %good values for initial balancing. Player tests are still required.
%\end{itemize}

The results of our experiments showed that the generation and value optimization for balancing of graph-based game economies with the proposed architecture is feasible. There are, however, several things that need to be discussed.

The generator is controllable in terms of the number and types of nodes and generated valid graphs in terms of the given constraints, showing an average validity of 97\%. Thereby, the median execution time of 25 ms is also fast. In comparison to~\cite{rogers_using_2023}, our implementation is also able to construct game economy graphs that do not only represent tree structures and therefore allow loops or contain probabilistics, for instance. This allows for greater precision and flexibility in modeling economies as described in~\cite{schreiber_game_2021,klint_micro-machinations_2013}.

We investigated on the general performance of the balancer by applying it to each economy in the generated dataset to a randomly chosen target value with a randomly chosen simulation length. 
The results (Table~\ref{tab:gen-performance}) vary greatly depending on the value of $\alpha$.
The best balanced proportion yields $\alpha=0.05$ with a share of 93.3\%. $\alpha=0.0$ allows no margin for the simulated target values, thus its results are worse. Also the execution time and needed generations differ per $\alpha$. Since the permissible margin of $\alpha=0.05$ allows for greater scatter, the target balance can be achieved faster and therefore its median generation and execution time are much faster compared two smaller $\alpha$.
However, there is no setting where all economy graphs could be balanced. In cases where the balancer improved overall, but could not achieve the expected quality, the algorithm may have gotten stuck in local optima.
Another problem is the challenge of balancing randomly selected combinations of pools and values in combination with the distribution and networking of different node types. For instance, there are cases in which a certain target value cannot be mathematically achieved within the randomly chosen simulation length.


%The result of 79.6\% of cases where the balancing criteria could be met compared with the initial fitness distribution (Figure~\ref{fig:res-balancing}) shows that the balancer is able to optimize the economies' weights accordingly for arbitrary values and number of simulation steps  within the tested range. However, the balancer failed in about a fifth of cases. Of the cases examined, 13.4\% represent instances where the balancer could enhance but fell short of the required fitness, and 7\% involved situations where no improvement occurred within the allowed number of generations. Further analysis suggests that some cases required more generations for successful termination, indicating challenges in balancing randomly chosen combinations of pools and values due to the distribution and interconnectedness of different node types.

With a case study of two fictional economies (mage and archer class), we delve into how the EA balances both to ensure equal damage output in the same time frame, addressing the objective in game balancing for diverse strategies and preventing a single dominant strategy from consistently prevailing.
We compare the results of two runs with two different values of $\alpha$, representing the threshold for values to consider as balanced. For both configurations, the balancer could find a solution within a short number of generations. A key finding here is that for the low value of $\alpha$ (0.01), the algorithm tries to minimize the fluctuation of values caused through randomness. While still the probabilities for normal and critical hits differ, it equalizes the damage for both hits and thereby mitigates the randomness. At the one hand, it fits the balancing criteria, at the other it might not be a desirable solution since now the intention of the economy design is obsolete. To address this shortcoming, we recommend to use low values of alpha only if randomness should have no or little impact. With other words, we can use $\alpha$ to not only configure the precision to the exact value, but also the influence of randomness.
For this case study we use the parametrization of the fitness function in Eq.~\ref{eq:f3} to balance two economies at once to a same value. In real world cases, however, often new game entities are embedded into an existing game ecosystem. Therefore, fitness function 1 can be used to balance the newly introduced content to a value which fits into the ecosystem.
Another point to mention here is, that due to the recursive execution of the economy framework, the mage's economy implements the play style of a spammer, using an ability whenever its cooldown is ready and enough mana available. Human players would also use other strategies, such as waiting for an ability that deals more damage even though another one is available. An interesting approach would be the implementation of small bots, each with different strategies in future work.

It was shown that the lightweight economy simulation framework is able to implement basic concepts of game economics on examples from the game Minecraft and two fictitious character classes. However, it lacks components to e.g., influence edge weights based on values of pools as implemented in~\cite{klint_micro-machinations_2013,vanrozen_adapting}. This would open up further opportunities to study more complex economies and other balancing objectives such as the counteracting of positive feedback loops.
Another limitation is that this research is based on simulations on an abstract game level. Since by design no real game is implemented and no humans for testing are involved, playtests are still required. It still depends on humans whether the generated economies with the computed weights are actually fun to play within the narrative setting chosen by the designer. Therefore, this research is intended to supporting the early stages of game design to find an interesting economy through generation and balancing initial values for the first player tests.
Lastly, evolutionary computing has a high dependency on randomness, especially in combination with probabilistics within the simulations. Hence we attempt to mitigate this by evaluating our method on a large sample of economies with a wide range of configuration values.

\section{Conclusion and Future Work}
We have proposed GEEvo (Game Economy Evolution), a framework consisting of two evolutionary algorithms (EAs) to generate and balance graph-based game economies using simulations.
In addition to a lightweight framework to simulate the economies for balancing, we introduced a fitness function which can be parameterized differently to balance economies towards various objectives. The results show that the EA for balancing can optimize the weights of economies to arbitrary values and simulation lengths. We further evaluated our method in a case study using fictional economies of two popular game character classes.
By looking exclusively at game economies from an abstract perspective, our method is independent of a specific game or genre and is intended to support designers in the early stages of development. 

For future work we aim to extend the EA for balancing towards handling multi-object evolution to fit on multiple balancing goals for an economy at once and extend the presented collection of fitness functions. In addition, we want to extend the simulation framework to handle more complex economies, e.g., to influence a weight edge depending on the value of a pool. This would open up interesting possibilities for investigating how positive feedback loops could to be counteracted by the EA. Furthermore, an investigation into the automated naming of an economy's nodes based on a given narrative context is of interest through recent advances in large language models (LLMs).

\label{sec:conclusion}
